Improving Attributed Text Generation of Large Language Models via Preference Learning

Large language models have been widely adopted in natural language processing, yet they face the challenge of generating unreliable content. Recent works aim to reduce misinformation and hallucinations by resorting to attribution as a means to provide evidence (i.e., citations). However, current attribution methods usually focus on the retrieval stage and automatic evaluation that neglect mirroring the citation mechanisms in human scholarly writing to bolster credibility. In this paper, we address these challenges by modelling the attribution task as preference learning and introducing an Automatic Preference Optimization (APO) framework. First, we create a curated collection for post-training with 6,330 examples by collecting and filtering from existing datasets. Second, considering the high cost of labelling preference data, we further propose an automatic method to synthesize attribution preference data resulting in 95,263 pairs. Moreover, inspired by the human citation process, we further propose a progressive preference optimization method by leveraging fine-grained information. Extensive experiments on three datasets (i.e., ASQA, StrategyQA, and ELI5) demonstrate that APO achieves state-of-the-art citation F1 with higher answer quality.

==> figures/analysis_po_compraison.tex <==
\begin{figure*}[hpt] % 使用 figure* 环境展示在同一行且跨列
\centering
\begin{minipage}{4.5cm}
\input{figures/fig_em_asqa}
\end{minipage}\hspace{2em}
\begin{minipage}{4.5cm}
\input{figures/fig_pre_asqa}
\end{minipage}\hspace{2em}
\begin{minipage}{4.5cm}
\input{figures/fig_rec_asqa}
\end{minipage}
\caption{ASQA} % 添加标题
\label{fig:asqa_preference_comparsion} % 添加标签用于引用
\end{figure*}


\begin{figure*}[hpt] % 使用 figure* 环境展示在同一行且跨列
\centering
\begin{minipage}{4.5cm}
\input{figures/fig_claim_eli5}
\end{minipage}\hspace{2em}
\begin{minipage}{4.5cm}
\input{figures/fig_pre_eli5}
\end{minipage}\hspace{2em}
\begin{minipage}{4.5cm}
\input{figures/fig_rec_eli5}
\end{minipage}
\caption{ELI5} % 添加标题
\label{fig:eli5_preference_comparsion} % 添加标签用于引用
\end{figure*}


==> tables/method_errors.tex <==
\begin{table*}[t]
\centering
\setlength\tabcolsep{2pt}
\small
\begin{tabular}{@{}ccp{8cm}@{}}
\toprule
\textbf{Error type}  & \textbf{Sub type} & \textbf{Description}\\ \midrule
\textbf{Irrelevant but supported} & - & The generated text is grounded on unhelpful reference documents. \\
\midrule
\multirow{3}{*}{\textbf{Relevant but unsupported}} & Hallucinated Statement & The generated text contains facts or information that can't be derived from the reference documents. \\ \cmidrule(lr){2-3}
                       & Mistaken Synthesis & Several reference documents are used, but facts or logics are mistakenly intermingled. The generated text thus contains factual error or logic error.\\ \cmidrule(lr){2-3}
                       & Unintentional Omission & The reference documents are used, but the key points are incomplete. There's no factual errors in generated text, but some information are omitted. \\
\bottomrule
\end{tabular}

\caption{Error types.}
\label{tab:error_types}
\end{table*}
